Hierarchical Categories in Colored Searching

In colored range counting (CRC), the input is a set of points where each point is assigned a ``color'' (or a ``category'') and the goal is to store them in a data structure such that the number of distinct categories inside a given query range can be counted efficiently. CRC has strong motivations as it allows data structure to deal with categorical data. However, colors (i.e., the categories) in the CRC problem do not have any internal structure, whereas this is not the case for many datasets in practice where hierarchical categories exists or where a single input belongs to multiple categories. Motivated by these, we consider variants of the problem where such structures can be represented. We define two variants of the problem called hierarchical range counting (HCC) and sub-category colored range counting (SCRC) and consider hierarchical structures that can either be a DAG or a tree. We show that the two problems on some special trees are in fact equivalent to other well-known problems in the literature. Based on these, we also give efficient data structures when the underlying hierarchy can be represented as a tree. We show a conditional lower bound for the general case when the existing hierarchy can be any DAG, through reductions from the orthogonal vectors problem.

==> conc.tex <==
We extended the colored counting problem to cases where the underlying
color set have some structure which we modelled either as a tree or a general
(sparse) DAG.
We showed that the hierarchical colored counting problem 
is at least hard as ordinary colored counting and thus the problem is 
hard for 2D and beyond. 

We gave an upper bound for the tree variant in 1D and through a series of reductions,
we showed that the generalized caterpillar version of HCC in 1D is equivalent to 2D weighted range counting (up to constant factors). 
Due to this and since 2D weighted range counting have not been improved for decades, the best known trade-off ($S(n)Q(n)=\Omega(n\log^2(n))$ 
is also a barrier for 1D HCC.

We showed the existence of a polynomial gap between the preprocessing time and the space complexity of the DAG variant in 1D.
This is one of the few instances in data structures where there exists such a gap between the preprocessing 
time and the space complexity. 

One possibility for future work is to improve the space complexity for tree HCC in 1D. 
Improving it by more than a $\log n$ factor would improve the long standing upper bound for 2D weighted range counting. 
On the contrary,  another open problem is to prove a lower bound trade-off for the tree HCC in 1D to show that it is 
truly harder than the generalized caterpillar.


